Extrapolating Multilingual Understanding Models as Multilingual Generators

Multilingual understanding models (or encoder-based), pre-trained via masked language modeling, have achieved promising results on many language understanding tasks (e.g., mBERT). However, these non-autoregressive (NAR) models still struggle to generate high-quality texts compared with autoregressive (AR) models. Considering that encoder-based models have the advantage of efficient generation and self-correction abilities, this paper explores methods to empower multilingual understanding models the generation abilities to get a unified model. Specifically, we start from a multilingual encoder (XLM-R) and propose a \textbf{S}emantic-\textbf{G}uided \textbf{A}lignment-then-Denoising (SGA) approach to adapt an encoder to a multilingual generator with a small number of new parameters. Experiments show that the proposed approach is an effective adaption method, outperforming widely-used initialization-based methods with gains of 9.4 BLEU on machine translation, 8.1 Rouge-L on question generation, and 5.5 METEOR on story generation on XLM-R$_{large}$. On the other hand, we observe that XLM-R is still inferior to mBART in supervised settings despite better results on zero-shot settings, indicating that more exploration is required to make understanding models strong generators.

==> 5_discussion.tex <==

\section{Qualitative Analysis -- What denoising brings}

% \subsection{Similarity between MLM and other generation tasks} \label{sec:mlm_head_discuss}


% In this section, we study why the masked language modeling classification head can be directly applied to generation tasks, and study the task similarity between masked language modeling and other generation tasks. Unlike iterative generation strategy we adopt in the question generation, we study translation tasks, since we can acquire very good performance with only one step generation. 

% We collect 1000 random sentences from each language direction in the TED dataset, and study the classification behavior between the MLM heads and AT models. for MLM head, we use the target sentence and adopt masked language modeling to acquire proposal for each token. For AT, we use translation. We can see that the similarity is shared between . 

% Therefore, we study such phenomena here to help the community have a clearer view

% We can see that English prediction have very similar. 



In this section, we provide a detailed qualitative analysis of various generation scenarios to study what difference the denoising technique makes in all three generation scenarios.

Table \ref{tab:denoise_analysis} presents what denoising brings in our model. For translation tasks, the 





% However, we have to give up the first language distribution.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/version_v1.png}
%     \caption{Distribution Graph}
%     \label{fig:distribution graph}
% \end{figure}

==> 7_prev_writing.tex <==
\section{Introduction}

% 先讲现状，causal models are dominant

\textcolor{red}{Current need of controllable text generation -> rethinking the role of bi-directional models and causal models -> current NAT success including diffusion -> no pretrained models for bi-directional generation models, why and do we need -> existing bi-directional understanding de-nosing pretraining based models already have very good ability of bi-directional generation, with simple PEFT methods can lead to good performance -> experiments on four kinds of generation.}


% plug and play should be high-lighted
With the current need for plug-and-play controllable text generation, causal models, including encoder-decoder architectures (mBART, mT5) and decoder-only architectures (GPT etc.), are often preferred, as we can easily control the generation behavior of these models by greedy sampling or nucleus sampling. Bidirectional understanding models, on the contrary, are often regarded as lacking of ability for high-quality generation and controllable text generation due to their inductive bias. 

But as can be implied by . Existing studies like initializing both the encoders and decoders from a pretrained multilingual are proven useful in boosting the downstream generation tasks, especially for translation. More interestingly, model initialized from mXLMR usually have better performance than mBART.

This prejudice is proven not true both theoretically and experimentally with recent success in non-auto-regressive generation\cite{savinov2021step}. On a variety of . This somehow presents the generation ability of bi-encoder models, meaning that bi-directional models can at least achieve comparable performance with regard to translation tasks. Beyond the machine translation tasks, with the current trend of diffusion methods including diffusion-LM and diffu-seq, bi-directional models are proven to be comparable with causal models.


% 所以一定要把understanding的问题解决 -- 其实还可以拉，我感觉效果不差的。
But still, no effective pretraining methods are found for these NAT methods. Only very limited number of works discuss the pretraining for NAT on summarization datasets. No pretraining paradigm for translation tasks are tried, especially when the parallel dataset is unavailable. 

A natural question that emerges would be, can existing pretrained multilingual models benefit all the downstream generation tasks? 

In this paper, we have found that existing bi-directional multilingual understanding models are already strong generators. Moreover, the ability of current understanding models may be far beyond our preconception of bi-directional models. Understanding is often regarded as the perquisite of creation. Therefore, pre-trained bi-directional understanding language models should also have the ability for high-quality generation. With the help of current PEFT methods including adapters, prefix tuning and prompt tuning, extremely small size of parameters can enable a high-quality plug-and-play multilingual translation model. With a plugger of approximately 8M parameters on each language pair, the pre-trained mXLMR-base can achieve comparable performance with transformer-big. Similar work includes MSP \cite{tan2022msp}, but they pretrain a totally new mGPT model for translation, while we simply use the current off-the-shelf mXLMR model, and achieve comparable performance.

Due to the fix of parameters and NAT's nature of lack for token dependency, the generation quality of the first phase is often noisy. Thanks to the de-noising pretraining strategies like Masked Language Modelling, understanding models can naturally cope with de-noising tasks. This enables an iterative de-nosing strategy for generation refinement, as most of the iterative non-auto-regressive translation methods favour.

The understanding nature also enables models with a strong ability for understanding-based generation tasks like Question-generation and Story-generation. On these tasks, transformers without pre-training fails because of overfitting. We then compare our models with mBART/mT5-based models. We still use the PEFT setting instead of full fine-tuning, and achieve comparable performance. This in turn shows the strong ability of understanding models.

Multilingual Understanding models can also support controllable generation tasks, controllable generation. Sentimental generation is blablabla. We can do that too. An example on SST5 can prove that.

Text-infilling tasks also well present the generation ability of bi-directional models, but this is something that causal models cannot achieve, as it can forecast what will occur in the next sentence or next paragraph ~ Need one tasks like this.

